A Dynamical Central Limit Theorem for Shallow Neural Networks

Recent theoretical works have characterized the dynamics of wide shallow neural networks trained via gradient descent in an asymptotic mean-field limit when the width tends towards infinity. At initialization, the random sampling of the parameters leads to deviations from the mean-field limit dictated by the classical Central Limit Theorem (CLT). However, since gradient descent induces correlations among the parameters, it is of interest to analyze how these fluctuations evolve. Here, we use a dynamical CLT to prove that the asymptotic fluctuations around the mean limit remain bounded in mean square throughout training. The upper bound is given by a Monte-Carlo resampling error, with a variance that that depends on the 2-norm of the underlying measure, which also controls the generalization error. This motivates the use of this 2-norm as a regularization term during training. Furthermore, if the mean-field dynamics converges to a measure that interpolates the training data, we prove that the asymptotic deviation eventually vanishes in the CLT scaling. We also complement these results with numerical experiments.

==> app-experiments.tex <==
\section{Additional Details of the Experiments}
\label{app.exper}
\subsection{Setup of the experiments reported in Section~\ref{sec.experiments}}
The numerical experiments reported in Figure~\ref{fig:results_main} are under the student-teacher setting, with both the student and the teacher being shallow neural networks. Both $\hat{D}$ and $\Omega$ are taken to be the unit sphere of $d=16$ dimensions, and we take $\hat{\varphi}(\zb, \xb) = \max(0, \langle \zb, \xb \rangle)$. The teacher network has two neurons, $(c_1, \zb_1)$ and $(c_2, \zb_2)$, in the hidden layer, with $c_1 = c_2 = 1$ and $\zb_1$ and $\zb_2$ sampled i.i.d. from the uniform distribution on $\hat{D}$ and then fixed across the experiments. We vary the width of the student network in the range of $m = 128, 256, 512, 1024$ and $2048$, with their $\zb$'s sampled i.i.d. from the uniform distribution on $\hat{D}$ and their $c$'s sampled i.i.d. from $\mathcal{N}(0, 1)$. We train the networks in the ERM setting, where we sample $n=32$ vectors i.i.d. from the uniform distribution $\nu$ on $\Omega$ as the training dataset, which then define the empirical data measure $\hat{\nu}(d \xb) = \frac{1}{n} \sum_{l=1}^n \delta_{\xb_l}(d \xb)$. We use the mean squared error as the loss function. 
We rescale both the squared loss and the gradient by $d$ in order to adjust to the $\frac{1}{d}$ factor resulting from spherical integrals. 
The models are trained for $20000$ epochs with learning rate (which is multiplied to the RHS of \eqref{eq:gd_particle}) set to be $1$.
For each choice of $m$, we run the experiment $\kappa=20$ times with different random initializations of the student network. The average fluctuation is defined as $\frac{1}{\kappa} \sum_{k=1}^\kappa \|f^{(m)}_k - \bar f^{(m)}\|_{\hat{\nu}}^2$ for the training loss and $\frac{1}{\kappa} \sum_{k=1}^\kappa \|f^{(m)}_k - \bar f^{(m)}\|_{\nu}^2$ for the exact population loss, with $\bar f^{(m)} = \frac{1}{\kappa} \sum_{k=1}^\kappa f^{(m)}_k$ being the averaged model, similar to the approach in \cite{geiger2019disentangling}. The other plotted quantities -- loss, TV-norm and $2$-norm -- are averaged across the $\kappa$ number of runs.



% The models are trained by performing GD on the exact population loss, where the loss and its gradients are computed analytically, both of which we rescale by $d$ in order to adjust to the $\frac{1}{d}$ factor resulting from spherical integrals. The models are trained for $20000$ epochs with learning rate (which is multiplied to the RHS of \eqref{eq:gd_particle}) set to be $1$.

\subsection{Additional experiments using the exact population loss}
\label{app:exper_pop}
In addition to the results shown in Figure~\ref{fig:results_main}, we also train the networks under the exact population loss
% and show the results in Figure~\ref{fig:results_pop}. 
In this setting, we optimize the student networks by gradient descent under the exact population loss where the data distribution $\nu$ is uniform on $\Omega$, which  
allows an analytical formula for the gradient using spherical integrals.
% , as we discuss in Appendix~\ref{app.mc_value}. 
In addition, besides the initialization scheme of the parameters discussed above, we also consider zero-initialization of the $c$ parameters.

% For each choice of $n$, we run the experiment $\kappa=20$ times with different random initializations of the student network. The average fluctuation is defined as $\frac{1}{\kappa} \sum_{k=1}^\kappa \|f^{(n)}_k - \bar f^{(n)}\|_{\hat{\nu}}^2$ for the training loss and $\frac{1}{\kappa} \sum_{k=1}^\kappa \|f^{(n)}_k - \bar f^{(n)}\|_{\nu}^2$ for the exact population loss, with $\bar f^{(n)} = \frac{1}{\kappa} \sum_{k=1}^\kappa f^{(n)}_k$ being the averaged model, similar to the approach in \cite{geiger2019disentangling}. The other plotted quantities -- loss, TV-norm and $2$-norm -- are averaged across the $\kappa$ number of runs.
% As a proof of concept, we optimize the student networks by gradient descent under the population loss where the data distribution is uniform on $\Omega$, which  
% allows an analytical formula for the gradient.
% % that greatly accelerates computations and provides an approximation for the empirical setting. 
% For each choice of $n$, we run the experiment $\kappa=20$ times with different random initializations of the student network. Detailed experimental setup and additional results for the ERM case and zero-initialization of the parameters are provided in Appendix \ref{app.exper}. The mean squared fluctuation is defined as $\frac{1}{\kappa} \sum_{k=1}^\kappa \|f^{(n)}_k - \bar f^{(n)}\|_{\nu}^2$, with $\bar f^{(n)} = \frac{1}{\kappa} \sum_{k=1}^\kappa f^{(n)}_k$ being the averaged model, similar to the approach in \cite{geiger2019disentangling}. The other plotted quantities -- loss, TV-norm and $2$-norm -- are averaged across the $\kappa$ number of runs.
\begin{figure}[!htb]
    \centering
    \includegraphics[scale=0.45,trim=15pt 0 0 0, clip]{figures/supplementary/o1_q=0.pdf} \\
    \vspace{-14pt}
    % \includegraphics[scale=0.38]{figures/thursday morning/o1init_nt=02_q=02_lambda=1e-02_run=05.pdf} \\
    \includegraphics[scale=0.45,trim=15pt 0 0 0, clip]{figures/supplementary/o1_q=2_lambda001.pdf} \\
    \vspace{-14pt}
    % \includegraphics[scale=0.38]{figures/thursday morning/zeroinit_nt=02_q=02_lambda=1e-02_run=05.pdf}
    \includegraphics[scale=0.45,,trim=15pt 0 0 0, clip]{figures/supplementary/zero_q=0.pdf}
     \vspace{-5pt}
    % \includegraphics[scale=0.53,trim=13pt 0 0 0, clip]{figures/friday morning/o1_q=0_internal.pdf} \\
    % \vspace{-8pt}
    
    % \includegraphics[scale=0.53,trim=13pt 0 0 0, clip]{figures/friday morning/o1_q=2_internal.pdf} \\
    % \vspace{-8pt}
    
    % \includegraphics[scale=0.53,,trim=13pt 0 0 0, clip]{figures/friday morning/zero_q=0_internal.pdf}
    %  \vspace{-5pt}
    \caption{Results of the numerical experiments described in Appendix~\ref{app:exper_pop}, where student networks of different widths are trained to learn teacher networks of width $2$ by performing gradient descent on the exact population loss. Each row corresponds to one setup. \emph{Row 1}: Using unregularized loss and non-zero initialization; \emph{Row 2}: Using regularized loss with $\lambda=0.01$ and non-zero initialization; \emph{Row 3}: Using unregularized loss and initialization. In each row, \emph{Panel 1} plots the trajectory of the neurons, $\thetab_i = (c_i, \zb_i)$, of a student network of width 128 during its training, with $x$-coordinate being the angle between $\zb_i$ and that of a chosen teacher's neuron and $y$-coordinate being $c_i$. The yellow dots, blue dots and cyan curves marking their initial values, terminal values, and trajectory during training. \emph{Panels 2-5} plot the average fluctuations (scaled by $m$), average loss, average TV norm, and average $2$-norm during training, respectively, computed across $\kappa=20$ runs with different random initializations of the student network for each choice of $m$. In \emph{Panel 2}, the \emph{solid} curves give the average fluctuation in the exact population loss and the black horizontal \emph{dashed} line gives the asymptotic Monte-Carlo bound in \eqref{eq:mcbound_lem33} computed in Appendix~\ref{app.mc_value} for this setting.
    In \emph{Panel 3}, the \emph{dotted} curve indicates the unregularized exact population loss, the \emph{dashed} curve the regularization term, and the \emph{solid} curve the sum of these two (i.e. total regularized loss). In \emph{Panels 4} and \emph{5}, the horizontal \emph{dashed} line gives the relevant norm of the teacher network.}
    % \caption{Results of numerical experiments, where student shallow neural networks of different widths are trained to learn teacher networks of width $2$. \emph{Row 1:} using unregularized square loss; \emph{Row 2:} using regularized square loss with $\lambda=0.01$. 
    % % \emph{Row 3}: Using regularized loss with $\lambda=0.01$ and zero initialization. 
    % In each row, panel 1 plots the trajectory of the neurons, $\thetab_i = (c_i, \zb_i)$, of a student network of width 128 during its training, with $x$-coordinate being the angle between $\zb_i$ and that of one of the teacher's neurons and $y$-coordinate being $c_i$. The yellow dots, blue dots and cyan curves mark their initial values, terminal values, and trajectory during training. Panels 2-5 plot the average fluctuation (scaled by $n$), average loss, average TV norm, and average $2$-norm during training, respectively, computed across $\kappa = 20$ runs with different random initializations of the student network for each choice of $n$. These quantities are defined in 
    % % Section \ref{sec.experiments}. 
    % Appendix~\ref{app.exper}.
    % In panel 2, the \emph{solid} curves give the average fluctuation in the \emph{training} loss, the \emph{dash-dot-dotted} curves give the average fluctuation in the \emph{exact population} loss computed analytically via spherical integrals, and the black horizontal \emph{dashed} line gives the asymptotic Monte-Carlo bound in \eqref{eq:mcbound_lem33} computed in Appendix~\ref{app.mc_value} for this setting.
    % In panel 3, the \emph{dotted} curves indicate the unregularized \emph{training} loss, the \emph{dashed} curves the regularization term, the \emph{solid} curves the sum of these two (i.e. the total regularized \emph{training loss}), and the \emph{dash-dot-dotted} curves the unregularized \emph{exact population loss}. In panels 4 and 5, the black horizontal \emph{dashed} line gives the relevant norm of the teacher network.}
    \label{fig:results_pop}
\end{figure}

The results are shown in Figure~\ref{fig:results_pop}. We observe that the mean squared fluctuations remain at a $1/m$ scaling with a general tendency to decay over time.
% , except for in the zero-initialization case, where an increase occurs in the first few epochs of training. 
In the unregularized case with non-zero initialization, the mean squared fluctuation decays at the same rate for different $m$ in roughly the first $10^3$ epochs, after which it decays faster for smaller $m$. Interestingly, this coincides with the tendency for student neurons with $\zb$ not aligned with the teacher neurons to slowly have their $|c|$ decrease to zero due to a finite-$m$ effect, which is also reflected in the decrease in TV-norm. Aside from this, the mean squared fluctuations decay at similar rates for different choices of $n$, which is consistent with our theory, since their dynamics are governed by the same dynamical CLT. 
Moreover, the values of the fluctuations for these choices of $m$ are indeed lower than the asymptotic Monte-Carlo bound given in \eqref{eq:mcbound_lem33} with $\mu_\infty$ and $f_\infty$ replaced by the target measure and function, whose analytical expression and numerical value in this setup are given in Appendix \ref{app.mc_value}.
We also see that the average loss values remain similar over time for different choices of $m$, justifying the approximation by a mean-field dynamics. Also, we notice that with either regularization or zero-initialization, the student neurons are aligned with one of the teacher neurons in both $\zb$ and $c$ after training, which then results in lower TV-norms and $2$-norms than using non-zero initialization and without regularization.


% The code is implemented in C++ and run on a cluster with single CPU. We take both $\Omega$ and $\hat{D}$ to be unit spheres of dimension $d = 16$. Both the student network and the teacher network are of the form \eqref{eq:basic}, with $\hat{\varphi}(\zb, \xb) = \max(0, \langle \zb, \xb \rangle)$ being the ReLU nonlinearity without bias. The teacher network has two neurons, $(c_1, \zb_1)$ and $(c_2, \zb_2)$, in the hidden layer, with $c_1 = c_2 = 1$ and $\zb_1$ and $\zb_2$ sampled i.i.d. from the uniform distribution on $\hat{D}$ and then fixed across the experiments. We vary the width of the student network in the range of $n = 128, 256, 512, 1024$ and $2048$, with their $\zb$'s sampled i.i.d. from the uniform distribution on $\hat{D}$ and their $c$'s sampled i.i.d. from $\mathcal{N}(0, 1)$. The models are trained by performing GD on the exact population loss, where the loss and its gradients are computed analytically, both of which we rescale by $d$ in order to adjust to the $\frac{1}{d}$ factor resulting from spherical integrals. The models are trained for $20000$ epochs with learning rate (which is multiplied to the RHS of \eqref{eq:gd_particle}) set to be $1$.

The code is implemented in C++ and run on a cluster with single CPU. For $n = 128, 256, 512, 1024$ and $2048$, the approximate running times of each run of $20000$ epochs are $1$ min, $2$ min, $8$ min, $30$ min and $150$ min, respectively.

The hyperparameter in regularization, $\lambda$, is manually selected from $0.01, 0.05$ and $0.1$. We select $0.01$ because it yields the best loss value (unsurprisingly) while also controlling the TV norm and the $2$-norm of the solution. Figure \ref{fig:other_lambdas} shows the same plots as the second row of Figure \ref{fig:results_pop} but with $\lambda = 0.05$ and $\kappa=10$ runs.

\begin{figure}[h]
    \centering
    % \includegraphics[scale=0.38]{figures/thursday morning/o1init_nt=02_q=00_lambda=0_run=05.pdf} \\
    % \includegraphics[scale=0.46,trim=13pt 0 0 0, clip]{figures/friday morning/o1_q=0_internal.pdf} \\
    % \vspace{-12pt}
    % % \includegraphics[scale=0.38]{figures/thursday morning/o1init_nt=02_q=02_lambda=1e-02_run=05.pdf} \\
    % \includegraphics[scale=0.46,trim=13pt 0 0 0, clip]{figures/friday morning/o1_q=2_internal.pdf} \\
    % \vspace{-12pt}
    % \includegraphics[scale=0.38]{figures/thursday morning/zeroinit_nt=02_q=02_lambda=1e-02_run=05.pdf}
    \includegraphics[scale=0.45,,trim=13pt 0 0 0, clip]{figures/supplementary/lambda=005.pdf}
    \caption{Same setup as the second row of Figure \ref{fig:results_pop}, except for $\lambda = 0.05$ instead of $0.01$.}
     \vspace{-5pt}
     \label{fig:other_lambdas}
\end{figure}


\subsection{Additional experiments with a non-planted target}
\label{app:nonp}
We also conduct an experiment in which the target function is not given by a teacher network. $\hat{D}$, $\Omega$, $\hat{\varphi}$ as well as the widths of the student networks remain the same as in the previous experiments. The target function is $f_*(\xb) = \int_{\hat{D}} \hat{\varphi}(\zb, \xb) \hat{\mu}_*(d \zb)$, where $\hat{\mu}_*$ is the uniform measure on the $1$-dimensional great circle in the first $2$ dimensions, i.e., $\{(\cos \theta, \sin \theta), 0, ..., 0: \theta \in [0, 2 \pi) \} \subseteq \mathbb{S}^d$. The student networks are trained using gradient descent under the exact population loss where the data distribution $\nu$ is uniform on $\Omega$, which  
allows an analytical formula for the gradient using spherical integrals, similar to the experiments in Appendix~\ref{app:exper_pop}.

The results are shown in Figure~\ref{fig:results_nonp}. We observe that the behavior of the fluctuations are similar to those found in Figure~\ref{fig:results_pop}.

\begin{figure}[h]
    \centering
    % \includegraphics[scale=0.38]{figures/thursday morning/o1init_nt=02_q=00_lambda=0_run=05.pdf} \\
    % \includegraphics[scale=0.46,trim=13pt 0 0 0, clip]{figures/friday morning/o1_q=0_internal.pdf} \\
    % \vspace{-12pt}
    % % \includegraphics[scale=0.38]{figures/thursday morning/o1init_nt=02_q=02_lambda=1e-02_run=05.pdf} \\
    % \includegraphics[scale=0.46,trim=13pt 0 0 0, clip]{figures/friday morning/o1_q=2_internal.pdf} \\
    % \vspace{-12pt}
    % \includegraphics[scale=0.38]{figures/thursday morning/zeroinit_nt=02_q=02_lambda=1e-02_run=05.pdf}
    \includegraphics[scale=0.45,,trim=13pt 28pt 0 0, clip]{figures/nonplanted2/nonp_unreg_o1init.pdf}
    \vspace{-14pt}
    \includegraphics[scale=0.45,,trim=13pt 0 0 0, clip]{figures/nonplanted2/nonp_unreg_zeroinit.pdf}
    \vspace{-14pt}
    \includegraphics[scale=0.45,,trim=13pt 0 0 0, clip]{figures/nonplanted2/nonp_unreg_zeroinit.pdf}
    \vspace{-14pt}
    \includegraphics[scale=0.45,,trim=13pt 0 0 0, clip]{figures/nonplanted2/nonp_reg001_zeroinit.pdf}
    \vspace{-5pt}
    \caption{Results of the experiments with a non-planted target using the exact population loss, as described in \ref{app:nonp}. \emph{Row 1}: Using unregularized loss and non-zero initialization; \emph{Row 2}: Using regularized loss with $\lambda=0.01$ and non-zero initialization; \emph{Row 4}: Using unregularized loss and zero initialization; \emph{Row 4}: Using regularized loss with $\lambda=0.01$ and zero initialization. In each row, \emph{Panel 1} plots the projection of the neurons' $\zb_i$ in the first two dimension. The other panels are under the same setting as Figure~\ref{fig:results_pop}.}
     \vspace{-5pt}
     \label{fig:results_nonp}
\end{figure}


==> app-long_time-prop.tex <==
\subsection{Proof of Lemma \ref{lem:34}}
\label{app:long_time-prop}
With $\mathfrak{D}_t$ defined in \eqref{eq:diff_term}, for \eqref{eq:mcbound_lem33} to hold, it is sufficient to show that 
\begin{equation}
    \lim_{T \to \infty} \fint_0^T \mathfrak{D}_t dt \leq 0~.
\end{equation}
Recall from \eqref{eq:diff_term_3_terms} that
\begin{equation}
    \begin{split}
        \fint_0^T \mathfrak{D}_t dt = - \frac{1}{T}\| \Tb_T \|_0^2 - 2 \fint_0^T \langle \Tb_t, \mathcal{A}_t^{(V)} \Tb_t \rangle_0 dt - \fint_0^T \langle \Tb_t, \mathcal{A}_t^{(K)} \Tb_t \rangle_0 dt~.
    \end{split}
\end{equation}
Since $\Tb_0 = 0$ and $\mathcal{A}_t^{(K)}$ is PSD, we see that the assumption \eqref{eq:T_t_ddV_cond} is sufficient.







==> sec-related.tex <==
\paragraph{Related Works:}
This paper continues the line of work initiated by \cite{mei2018mean, chizat2018global, rotskoff2018parameters, sirignano2018dgm} that studies optimization of over-parameterized shallow neural networks under the mean-field scaling.
Global convergence for the unregularized setting is discussed in \cite{mei2018mean,mei2019mean,sirignano2018dgm,rotskoff2018parameters}.
In the regularized setting, \cite{chizat2018global} establishes global convergence in the mean-field limit under specific homogeneity conditions on the neuron activation.
Other works that study asymptotic properties of wide neural networks include \cite{ghorbani2019limitations, geiger2019disentangling, bai2019beyond, dyer2019asymptotics, hanin2019finite, huang2019dynamics, woodworth2020kernel, luo2020phase, adlamneural}, notably investigating the transition between the so-called \emph{lazy} and \emph{active} regimes \cite{chizat2019lazy}, corresponding respectively to linear versus nonlinear learning. Our focus is on the dynamics under the mean-field scaling, which encompasses the active, nonlinear regime. 

A relevant work concerning the sparse optimization of measures is \cite{chizat2019sparse}, where under a different metric for gradient flow and additional assumptions on the nature of the minimizer, it can be established that fluctuations vanish for sufficiently large $n$. 
Our results are only asymptotic in $n$ but apply to broader settings in the context of shallow neural networks.
Concerning the next-order deviations of finite neural networks from their mean-field limit, \cite{rotskoff2018parameters} show that the scale of fluctuations is below that of MC resampling for unregularized problems using non-rigorous arguments. \cite{sirignano2020mean} provides a CLT for the fluctuations at finite time under stochastic gradient descent (SGD) and proves that the fluctuations decay in time in the case where there is a single critical point in the parameter space. Our focus is on the long-time behavior of the fluctuations in more general settings. Another relevant topic is the propagation of chaos in McKean-Vlasov systems, which study the deviations of randomly-forced interacting particle systems from their infinite-particle limits \citep{braun1977vlasov, sznitman1991topics, spohn2012large, baladron2011mean}. In particular, a line of work provides uniform-in-time bounds to the fluctuations in various settings \citep{del2000branching, cortez2016uniform, salem2018gradient, salhi2018uniform, durmus2018elementary}, but the conditions are not applicable to shallow neural networks. Concurrently to our work, \cite{de2020quantitative} studies quantitative propagation of chaos of shallow neural networks trained by SGD, but the bound grows exponentially in time, and therefore cannot address the long-time behavior of the fluctuations.

Learning with neural networks exhibits the phenomenon that generalization error can decrease with the level of overparameterization \citep{belkin_reconciling_2019, spigler2018jamming}. \cite{neal2018modern} proposes a bias-variance decomposition that contains a variance term initialization in optimization. They show in experiments that this term decreases as the width of the network increases, and justifies this theoretically under the strong assumption that model parameters remain Gaussian-distributed in the components that are irrelevant for the task, which does not hold in the scenario we consider, for example. \cite{geiger2020scaling} provides scaling arguments for the dependence of this term on the width of the network. Our work provides a more rigorous analysis of the dependence of this term on the width of the network and training time.






